Heavy neutrinos: The chosen ones to bring balance to physics

The Standard Model of Particle Physics has proven to be tremendously successful as the fundamental theory that describes the elementary particles that compose our Universe, as well as the interactions among them. Despite the countless experimental results that have ratified the theoretical predictions of this model, there are sound reasons to think it must be extended. Some are rather theoretical, while others are due to the observation of certain phenomena that the the Standard Model cannot explain. Chief among the latter is the massive nature of neutrinos, the most elusive particles in the Universe, which are rendered massless by the Standard Model. This contradiction establishes the starting point of this PhD thesis, which discusses the role of heavy neutrinos (a hypothetical new type of neutrino) as responsible of generating the mass of the observed neutrinos. Certain extensions of the Standard Model will be explored, which include these new particles and offer common solutions to neutrino masses and to other open problems. The consequences of the interactions of these new neutrinos with Standard Model particles will also be studied, as well as how they can be characterized by the means of present and future experimental observations.

==> custom_commands.tex <==
%%%%%%%%%% A FEW SHORTCUTS %%%%%%%%%%%%%
\newcommand{\marrow}[5]{%
    \fmfcmd{style_def marrow#1
    expr p = drawarrow subpath (1/4, 3/4) of p shifted 6 #2 withpen pencircle scaled 0.4;
    label.#3(btex #4 etex, point 0.5 of p shifted 6 #2);
    enddef;}
    \fmf{marrow#1,tension=0}{#5}}

% \newcommand{\refeq}[1]{Eq.~(\ref{#1})}
\newcommand{\refeqs}[2]{Eqs.~(\ref{#1})~and~(\ref{#2})}
\newcommand{\refeqss}[3]{Eqs.~(\ref{#1}), (\ref{#2})~and~(\ref{#3})}
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\reffigs}[2]{Figs.~\ref{#1}~and~\ref{#2}}
\newcommand{\refsec}[1]{Section~\ref{#1}}
\newcommand{\refapp}[1]{Appendix~\ref{#1}}
\newcommand{\reftab}[1]{Table~\ref{#1}}
\newcommand{\refref}[1]{Ref.~\cite{#1}}
\newcommand{\refrefs}[2]{Refs.~\cite{#1}~and~\cite{#2}}
\newcommand{\ewsb}{\ensuremath{\slashed{\text{EW}}}}
\newcommand{\breakEW}{\ensuremath{\xrightarrow{\ewsb}}}

\newcommand{\EFM}[1]{\textcolor{blue}{{ [EFM: \bf #1]}}}


\def\abelian{abelian}
\def\nonabelian{non-abelian}
\def\lagrangian{lagrangian}
\def\eg{\emph{e.g.}}
\def\ie{\emph{i.e.}}
\def\aka{\emph{a.k.a.}}
\def\muboone{MicroBooNE}
\def\icarus{Icarus}
\def\minerva{MINER$\nu$A}
\def\anu{\overline{\nu}}
\newcommand{\sinc}{\ensuremath{\text{sinc}}}
\newcommand{\unit}{1\!\!1}

\def\mphi{m_{\Phi}}
\def\mhiggs{m_{H}}
\def\lphi{\lambda_{\Phi}}
\def\lhiggs{\lambda_{H}}
\renewcommand{\phi}{\varphi}

%%%%%%% A few editorial macros. %%%%%%%
\newcommand{\lorem}{ \textcolor[rgb]{0.8,0.8,0.8}{Grandeur pious ocean virtues depths virtues. Prejudice enlightenment depths selfish contradict decieve. Ultimate inexpedient war eternal-return zarathustra strong insofar society ocean philosophy battle snare zarathustra derive. Christianity salvation dead ultimate hope law pinnacle fearful morality evil disgust. Victorious society burying of morality sea ultimate law.}}

\newcounter{CommentCount}
\setcounter{CommentCount}{1}

\newcommand{\marcom}[2]{\textsuperscript{\textcolor{#1}{\theCommentCount}}\marginpar{\textsuperscript{\textcolor{#1}{\theCommentCount}}\textcolor{#1}{{\small#1: #2}}}\stepcounter{CommentCount}}

\newcommand{\newtext}[2]{\textcolor{#1}{\ul{#2}}}

%%%%%%%%%%%%%% TABLES 
\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type

%%%%%%%%%%%%%% GROUP EDITING 
% Add your own colour down here 
\newcommand{\mh}[1]{\textcolor{purple}{MH: #1}}
\newcommand{\mhdel}[1]{\textcolor{purple}{\sout{#1}}}
\definecolor{jhg}{rgb}{0.984314,0.145098,0.462745}
\newcommand{\JHG}[1]{\textbf{\textcolor{jhg}{JHG: #1}}}
\newcommand{\gitlink}{\href{https://github.com/mhostert/Heavy-Neutrino-Limits}{\textsc{g}it\textsc{h}ub {\large\color{blue-violet}\faGithub}}}


